Robust Product Markovian Quantization

Recursive marginal quantization (RMQ) allows the construction of optimal discrete grids for approximating solutions to stochastic differential equations in d-dimensions. Product Markovian quantization (PMQ) reduces this problem to d one-dimensional quantization problems by recursively constructing product quantizers, as opposed to a truly optimal quantizer. However, the standard Newton-Raphson method used in the PMQ algorithm suffers from numerical instabilities, inhibiting widespread adoption, especially for use in calibration. By directly specifying the random variable to be quantized at each time step, we show that PMQ, and RMQ in one dimension, can be expressed as standard vector quantization. This reformulation allows the application of the accelerated Lloyd's algorithm in an adaptive and robust procedure. Furthermore, in the case of stochastic volatility models, we extend the PMQ algorithm by using higher-order updates for the volatility or variance process. We illustrate the technique for European options, using the Heston model, and more exotic products, using the SABR model.

==> Figures/Tikz_regions.tex <==
\begin{tikzpicture}

\draw [thick] (1,1.5) rectangle (3.5,3);
\draw [->, thick] (0,0.5) -- (4.5,0.5);
\draw [->, thick] (0,0.5) -- (0,4);
\draw [dashed, thick] (0,3) -- (4.5,3);
\draw [dashed, thick] (0,1.5) -- (4.5,1.5);
\draw [dashed, thick] (1,0.5) -- (1,4);
\draw [dashed, thick] (3.5,0.5) -- (3.5,4);
\draw [fill] (2.25,2.25) circle [radius=0.05];
\draw [fill] (1,3) circle [radius=0.05];
\draw [fill] (3.5,3) circle [radius=0.05];
\draw [fill] (1,1.5) circle [radius=0.05];
\draw [fill] (3.5,1.5) circle [radius=0.05];

\node at (1,0) {$x^{(1),\,j-}_{k+1}$};
\node at (3.5,0) {$x^{(1),\,j+}_{k+1}$};
\node at (-0.75,1.5) {$x^{(2),\,v-}_{k+1}$};
\node at (-0.75,3) {$x^{(2),\,v+}_{k+1}$};
\node [above] at (2.25,2.25) {$(x^{(1),\,j}_{k+1}, x^{(2),\,v}_{k+1})$};
\node [right] at (4.5,0.5) {$\Gamma^{(1)}_{k+1}$};
\node [above] at (0,4) {$\Gamma^{(2)}_{k+1}$};

\end{tikzpicture}

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DEFINITION: \widebar
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[textsize=footnotesize]{todonotes}
%\newcommand{\todo}[1]{}
%\renewcommand{\normalmarginpar}{}
%\renewcommand{\reversemarginpar}{}
\usepackage{amsfonts}                                 	% Provides \mathbb
\usepackage{mathrsfs}									% Provides \mathscr
\usepackage{mathtools}									% Provides \prescript, \DeclarePairedDelimiter, \vcentcolon

\newcommand{\R}{\mathbb{R}}                         	% Reals
\renewcommand{\P}{\mathbb{P}}                       	% Real-world probability
\newcommand{\sigalg}[1]{\mathscr{#1}}               	% Sigma algebra
\newcommand{\F}{\sigalg{F}}                         	% Sigma algebra F
\newcommand{\triple}{(\Omega,\F,\P)}                	% Probability triple
\newcommand{\ind}[1]{\mathbb{I}_{\left\{#1\right\}}}	% Indicator function

\renewcommand{\b}{\mathbf}                              % Bold mathematics
\newcommand{\bx}{\mathbf{x}}                            % Vector x
\newcommand{\bX}{\mathbf{X}}                            % Vector X
\newcommand{\Xq}{\widehat{X}}                           % Quantized X
\newcommand{\bXq}{\widehat{\bX}}                        % Quantized vector X
\newcommand{\Xd}{\widebar{X}}                           % Discretized X
\newcommand{\bXd}{\widebar{\bX}}                        % Discretized vector X
\newcommand{\Xa}{\widetilde{X}}							            % Approximate X
\newcommand{\bXa}{\widetilde{\mathbf{X}}}		            % Approximate vector X
\newcommand{\bxq}{{\b{x}}}
\newcommand{\Yq}{\widehat{Y}}           				        % Quantized Y
\newcommand{\Yd}{\widebar{Y}}                           % Discretized Y 
\newcommand{\Ya}{\widetilde{Y}}                         % Approximate Y

\newcommand{\bGamma}{\mathbf{\Gamma}}					          % Column-vector of codewords
\newcommand{\U}{\mathcal{U}}							              % Update function
\newcommand{\rcoloneqq}{=\vcentcolon}		              	% right colon equals

\DeclarePairedDelimiter\norm{\lvert}{\rvert}	          % Euclidean norm | Absolute value | Cardinality (Resize with *)
\DeclarePairedDelimiter\Ebraces{[}{]}
\DeclarePairedDelimiter\Pbraces{(}{)}
\DeclarePairedDelimiterX\cEbraces[2]{[}{]}{#1 \;\delimsize\vert\; #2\,}
\DeclarePairedDelimiterX\cPbraces[2]{(}{)}{#1 \;\delimsize\vert\; #2\,}
\newcommand{\E}{\mathbb{E}\Ebraces}				              % Expectation (Resize with *)
\newcommand{\Prob}{\mathbb{P}\Pbraces}			            % Probability of an event (Resize with *)
\newcommand{\cE}{\mathbb{E}\cEbraces}			              % Conditional expectation (Resize with *)
\newcommand{\cProb}{\mathbb{P}\cPbraces}		            % Conditional Probability (Resize with *)

\newcommand{\dx}[2]{#1'(#2)}                          % Derivative wrt x
\newcommand{\ddx}[2]{#1''(#2)}							          % Second derivative wrt x


%\newcommand{\iset}{\mathcal{I}}
\newcommand{\iset}{i}
%\newcommand{\ivec}{\iota}
\newcommand{\ivec}{i}

% Notational changes

\newcommand{\n}{n}                      % n-th component of SDE
\newcommand{\nsup}{\n}                  % superscript of nth component
\newcommand{\gensup}[1]{#1}             % general superscript
\newcommand{\iseta}[1]{{\iset}_{#1}}
\newcommand{\icart}{\mathcal{I}}
\newcommand{\icarta}[2]{\icart_{#1}^{#2}}

\newcommand{\red}[1]{{\color{red}{#1}}}
